On the nature of the boundary resonance error in numerical homogenization and its reduction

Numerical homogenization of multiscale equations typically requires taking an average of the solution to a microscale problem. Both the boundary conditions and domain size of the microscale problem play an important role in the accuracy of the homogenization procedure. In particular, imposing naive boundary conditions leads to a $\mathcal{O}(\epsilon/\eta)$ error in the computation, where $\epsilon$ is the characteristic size of the microscopic fluctuations in the heterogeneous media, and $\eta$ is the size of the microscopic domain. This so-called boundary, or ``cell resonance" error can dominate discretization error and pollute the entire homogenization scheme. There exist several techniques in the literature to reduce the error. Most strategies involve modifying the form of the microscale cell problem. Below we present an alternative procedure based on the observation that the resonance error itself is an oscillatory function of domain size $\eta$. After rigorously characterizing the oscillatory behavior for one dimensional and quasi-one dimensional microscale domains, we present a novel strategy to reduce the resonance error. Rather than modifying the form of the cell problem, the original problem is solved for a sequence of domain sizes, and the results are averaged against kernels satisfying certain moment conditions and regularity properties. Numerical examples in one and two dimensions illustrate the utility of the approach.

==> computational_cost2d.tex <==
The computational cost associated to reducing the cell resonance error is now
analyzed in the case of periodic media in dimension $d>1$. Several cases are
considered, namely: (i) solving a single, unmodified, elliptic problem (the ``naive" 
case analyzed in \cite{pingbingming:2004}); (ii) solving a single elliptic problem
that includes a zeroth order term, analyzed in \cite{gloria:2011}; (iii) solving 
a time-dependent hyperbolic problem, analyzed in \cite{runborg:2016}; and (iv) 
solving a sequence of unmodified elliptic problems, analyzed in the present work.
It is assumed that \cref{thm:1d_err_thm} proven in \cref{sec:1d_err_proof} generalizes to higher
dimensions, as suggested by the numerical examples in \cref{sec:numerical_results2d}. 

Assume that a linear system with $N$ degrees of freedom can be solved
with computational cost proportional to $N^{\alpha}$. For example, $\alpha = 3$ for
straightforward LU decomposition, or $\alpha=2\, (2.5)$ for a direct method 
that takes advantage of the sparsity that results from the discretization of an elliptic 
operator in two or three dimensions. In an ideal scenario, $\alpha=1$ could be achieved with 
multigrid; however, for microscopic domain length $\eta$ sufficiently large
relative to $\epsilon$, it is not clear that a multigrid iteration will converge
since the course grids will not be able to resolve the oscillatory nature of the solution. 
Lastly, because the microscale problems are typically posed with 
periodic boundary conditions on squares/cubes, 
one can use pseudo-spectral methods, which has the advantage of quasi-optimal complexity for the case
of an analytic tensor $a^{\epsilon}$, see \cite{abdulle:2007}. 
Furthermore, assume that the cost of estimating the homogenized coefficients,
using a quadrature formula for instance, given the solution to the microscale
problem, is dominated by the cost of the linear solve necessary to obtain the solution. 
In all cases, let $\tau$ denote some fixed error tolerance for the cell resonance error. 

For an elliptic microsolver, the number of degrees of freedom is proportional to 
$(\eta/\epsilon)^d$; hence, the total computational cost is proportional to 
$(\eta/\epsilon)^{\alpha d}$. The strategy proposed in the present work requires solving
a sequence of elliptic problems on domains with lengths that range from $\eta$ to
$2\eta$ in order to approximate $\rho^{\epsilon}$. 
Since $\rho^{\epsilon}$
can oscillate with period $\epsilon$, in general $\eta/\epsilon$ elliptic solves are required,
each of which cost $(\eta/\epsilon)^{\alpha d}$. \red{For the hyperbolic solver...}
 
The total computational cost associated to reducing the the cell resonance error below 
some tolerance $\tau$ is summarized
 in table \ref{table:cost_analysis}. The cost is a function of  
dimension $d$, linear solver complexity $\alpha$, and the order of the boundary error reduction strategy
for the cases (i)-(iv) above. 

\begin{center}
\emph{maybe make this paragraph part of the conclusion. just add a rehash of the abstract/intro. 
also maybe add again citations to the masmoudi and feldman papers and say that's future work. }
\end{center}

It is important to to note that in any serious application that requires the use of numerical homogenization, 
the performance of the microsolver at relatively low values of $\eta$ determines
its utility; depending on the application, this could mean $\eta$ is several 
times the assumed period, or correlation length, $\epsilon$ of the heterogeneous media. 
The cost estimates in table \ref{table:cost_analysis} assume the asymptotic 
rates of the proposed methods have been reached, which might not be true
until $\eta = \mathcal{O}(10\epsilon)$ or larger. 
A comparison of the existing numerical homogenization methods proposed 
in the literature at such ``practical" values of $\eta$ is beyond the scope
of the present work. We believe that such a study, especially if conducted 
in collaboration with researchers in the engineering community, is likely to 
be valuable to streamline research in numerical homogenization.
In addition, serious applications of numerical homogenization are most likely implemented in a 
high-performance computing environment in which 
effective use of parallelization strategies is crucial. 
Hence, this is also an important factor for practitioners to consider
when selecting a multiscale computational strategy. 
\begin{table}
  \begin{center}
  %\def~{\hphantom{0}}
    \begin{tabular}{c c c c}
     Micro problem                & Computational cost             & Error             & Cost for a tixed tolerance    \\
    \hline
    Unmodified elliptic           & $(\eta/\epsilon)^{\alpha d}$                   & $\epsilon/\eta$     & $\tau^{-\alpha d}$  \\
    Elliptic w/ zeroth order term & $(\eta/\epsilon)^{\alpha d}$                   & $(\epsilon/\eta)^4$ & $\tau^{-\alpha d/4}$ \\
    Sequence of elliptic problems & $\eta/\epsilon\cdot(\eta/\epsilon)^{\alpha d}$ & $(\epsilon/\eta)^s$ & $\tau^{-(\alpha d +1)/s}$\\
    Hyperbolic                    &   \red{?}                      & $(\epsilon/\eta)^q$ & \red{?}  \\
    \hline
    \end{tabular}
    \caption{Comparison of the computational cost associated to reducing the cell resonance error below
    some fixed tolerance for some of the microscale problems proposed in the literature. 
    Here $s = \min\{p+1,q+2\}$ for averaging kernel $K \in \mathbb{K}^{-p,q}$. The averaging kernels in 
    the hyperbolic solver from \cite{runborg:2016} are defined slightly differently than those in the
    present work, but the meaning of $q$ is identical.}
  \label{table:cost_analysis}
  \end{center}
\end{table}








